ReLoRA: High-Rank Training Through Low-Rank Updates

Despite the dominance and effectiveness of scaling, resulting in large networks with hundreds of billions of parameters, the necessity to train overparameterized models remains poorly understood, while training costs grow exponentially. In this paper, we explore parameter-efficient training techniques as an approach to training large neural networks. We introduce a novel method called ReLoRA, which utilizes low-rank updates to train high-rank networks. We apply ReLoRA to training transformer language models with up to 1.3B parameters and demonstrate comparable performance to regular neural network training. ReLoRA saves up to 5.5Gb of RAM per GPU and improves training speed by 9-40% depending on the model size and hardware setup. Our findings show the potential of parameter-efficient techniques for large-scale pre-training.

==> tables/optimizer_reset_ablations.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccc}
\toprule
Reset type & Amount of reset & Perplexity ($\downarrow$) \\
\midrule
No reset       & 0\%   & ?? \\
Full reset     & 100\% & ?? \\
Random pruning & ??small number like 50    & N/A \\
Random pruning & 90\%    & N/A \\
Random pruning & 99\%    & N/A \\
Magnitude pruning & ??small number like 50    & N/A \\
Magnitude pruning & 90\%    & N/A \\
Magnitude pruning & 99\%    & N/A \\
\bottomrule
\end{tabular}
\caption{Ablation studies of optimizer reset types.}
\label{tab:ablaitons}
\end{table}


==> tables/restart_frequency.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccc}
\toprule
Restart & Perplexity ($\downarrow$) \\
\midrule
0 (No restarts)     & ?? \\
500       & ?? \\
1000      & ?? \\
2500      & ?? \\
5000      & ?? \\
\bottomrule
\end{tabular}
\caption{Restart frequency effects. We'll need to convert this into a plot. It shouldn't be a table.}
\label{tab:ablaitons}
\end{table}

